Fast Sequence Component Analysis for Attack Detection in Synchrophasor Networks

Modern power systems have begun integrating synchrophasor technologies into part of daily operations. Given the amount of solutions offered and the maturity rate of application development it is not a matter of "if" but a matter of "when" in regards to these technologies becoming ubiquitous in control centers around the world. While the benefits are numerous, the functionality of operator-level applications can easily be nullified by injection of deceptive data signals disguised as genuine measurements. Such deceptive action is a common precursor to nefarious, often malicious activity. A correlation coefficient characterization and machine learning methodology are proposed to detect and identify injection of spoofed data signals. The proposed method utilizes statistical relationships intrinsic to power system parameters, which are quantified and presented. Several spoofing schemes have been developed to qualitatively and quantitatively demonstrate detection capabilities.

==> MeetingNotes.tex <==

\section{Notes from 4/24 planning meeting}

\begin{enumerate}
\item Hard limit - 8 pages
\item 5/1 open for submission
\item 8/31 deadline
\item gray scale for R plots, rather than color? Or note, ``color online''
\end{enumerate}

\begin{itemize}
\item Spoofed data. Tony interested in seeing spoofing only based on time.

\begin{enumerate}
\item (done) current method: mirroring 
\item (done, as drift) time skew.  Add a few seconds, minutes?  
\item (done) clock drift - undersample for a period of time
\item (done) Rickie's spoofing method - prediction function
\end{enumerate}
\item (nope) spoofing multiple PMUs?
\item (done) Machine learning detection tasks: use 2 or 3
\begin{enumerate}
\item (done) Rickie's preliminary result (high true (+) with some false (+)
\item (nope) Multi-PMU approach?
\item 
\end{enumerate}
\item How to evaluate the detection?  What are the metrics?
\begin{enumerate}
\item From Rich, this paper - MCD and MCOOB
\item Time it takes to detect a spoofing event
\item (done: FDR) Number of false positives in ratio 
\item Evaluate noise?  Spectrum should shift once spoof initiates.  Look at noise color.  Conduct wavelette (segmented FFT) on our R values. Faster than observing a roll-off on R values?? 
\end{enumerate}
\item Data sets
\begin{enumerate}
\item Use WSU-V archive data
\item Use OSU PMU hardware (3 + 2 not so healthy)
\end{enumerate}
\item PNNL finding - PMU noise is not white.
\item BPA has changed security classifcation of data.  Perhaps cannot get new data?
%\begin{itemize}
\item Timeframe
\begin{enumerate}
\item Develop spoof data sets:    
\item OSU - getting OSU PMU data from campus h/w: 5/1 - 5/21 
\item Rich to eval R noise evaluation: 5/1 - 5/21 
\item OSU to prep time-skew data sets: 5/1 - 5/21 
\item WSU Run ML algorithms 1st round: 5/1 - 5/21 - 1st set of results
\item group meeting around 5/21
\item evaluation \& analysis: 5/14 - 6/1
\item Run ML algorithms 2nd round \textit{if needed}: 6/1 - 6/21
\item Writing: 5/1 - 7/1
\end{enumerate}
\end{itemize}

\section{Notes from 5/15 meeting}

\begin{enumerate}
\item 
\begin{enumerate}
\item Rickie's results. normal - $>$ 95\%, 85\% spoofed data $<$ 90\%
\item Rickie - time scale spoofing, poly spoofing, mirror spoofing, statistical random walk
\item support vector machine (SVM)
\item See Rickie's notebook
\item Analysis needed
\item Need to rerun using: (1) voting scheme for existing classifiers; and ideally (2) a single classifier for all spoof types.
\end{enumerate}
\item Note can run multiple detectors that have been trained with different classifiers.  Using voting to determine when detectors are in agreement.
\item wavelet decomposition - contain some valuable info that may enhance detection.  Noise level and envelope in wavelet vectors increases after spoof starts.
\item decomposition removes noise
\item include wavelet decomp into this paper? - no, let's consider as future work.  
\begin{enumerate}
\item Re-runs - voting scheme? yes (5/15-6/1)
\item writing 5/15-6/30:
\begin{enumerate}
\item Expand spoofing methods discussion (3 of 4).  Use all 5?  No (nix random walk, timescale 1/2 (b/c approach is different). Use \textbf{timescale (2/3, 3/4, \dots)}, \textbf{mirror}, \textbf{polynomial}) 5/15 - 6/1
\item Re-run - use single classifier? not yet
\item evaluation \& analysis: 5/15 - 6/14
\item OSU - discuss \textbf{how} data could be spoofed in h/w. 5/15-6/1
\item conclusion, final edits, 6/14 - 6/30
\end{enumerate}

\begin{enumerate}
\item re-read!!
\item describe SVM (short), training procedure, features.
\item testing results
\item analysis
\item Use OSU h/w data? Probably not enough data to be useful. Not enough PMUs for correlation.
\end{enumerate}
\end{enumerate}
\end{enumerate}


\section{Notes from 5/28}

\begin{enumerate}
\item OSU - paragraph discussing how data could be spoofed in h/w. \hl{Done. Found recent work that shows how to do this with the GPS signal} 
\item SVM description (short)
\item Look at code - spoof window correct (red lines)?  Spoof starts at 1800 -- (SW: I don't think so. 1st red line is at 1650 for 300 cycle spoof, 1740 for 120 cycle spoof; both end 2 windows later -- however, in both cases, I think the first red line should be at 1800 and the second should be one window length later).
\item In Figure 2 caption, note what the red lines mean?  Note is an example mirror spoof.
\item (future) Number of support vectors matter?  Results conclusive enough to include?  Let's not. Avenue for follow up paper: explore complexity of decision surface as function of feature count.
\item Ok with results to date? 
\item (done) Include plots for other spoof types?  Yes, use a time-dilation example. Side-by-side Figure 3 (spf1) with another figure (spf8, time-dilation).
\item Write up conclusion.
\item And an abstract! 
\item Advance the timeline to finish by 6/14
\begin{enumerate}
\item Regenerate Figure 1 - better resolution (goto 600 dpi) - Bob.  Font consistency.  Send data to Jordan so he can generate Figure and make it consistent with other Figures.  Use default python font settings. Use cycles on the x -axis.  (JL: Done - added line styles for BW print. \hl{Comments?})
\item Ok with color figures?  Print in BW by default (else pay extra), online in color.  Save as png and eps w/ 600 dpi (JL: Resolution of Figure 1 on par with others -- is this still needed?)
\item Jordan: convert other figures to eps.  Need eps and png for all Figures. (JL: Converted to .eps except Spoof1\_minute1\_freq\_300 [pending comments given in caption])
\end{enumerate}
\item Meet again on 6/17, 9:30am.
\end{enumerate}

\section{Notes from 6/17}

\begin{itemize}
\item Fig 2, dotted red lines. Should begin at the same time, 1/2 way through the 1 minute period, 1800.
\item Need eps generation for Figure 2?
\item Need more to describe SVM
\item Need conclusion
\item Still have ~1 page.  Could show more detailed Fig 3:  
    \begin{itemize}
    \item Add another parameter, or <--- Do this one, negative sequence phase 
    \item another minute of data 
    \end{itemize}
\item All: need to read through
\end{itemize}

\section{Notes from 6/26}

\begin{itemize}
\item (a) (b) labels missing from Fig 4 (fixed)
\item section 4 MCOOB, MCD - what do we do with this? Tie in to use of SVM?  Drop it?  Use as strawman?  Eduardo to add section tying these into SVM.
\item ECS to expand on how GPS attacks can be done - literature references 20, 21, 22
\item fix capitals in bibtex - Jordan
\item Xinghui - add comments (within section VB or conclusion?) regarding generalizability
\item Scott working on re-running SVM Re: fix to Rickie's code (Fig 4)
\item results will affect voting ensemble, Table IV 
\item Scott wants to run SVM using the features identified in the intra-PMU correlations (V+ mag, V+ angle, f)
\item Need conclusion, but wait till new set of results is in.
\item Move on to NSF of BPA TI?  BPA April 16.  Applicable NSF FOAs?
\item meeting 7/1 9:30am
\end{itemize}

\section{Notes from 7/1}

\begin{itemize}
\item Declaire ``Spoof Window'' when window has one or more element OR ``Spoof Window'' when window has 50\% spoofed elements.  Go with the latter.  We've shown the trade-off between latency Show with the x2 and x3/2 cases only (need new table).
\item 3-feature vs 5-feature: performance is not as good with 3-features when using the ``new'' method.  Rerun with ``Old'' method.  
\item Remove Intra-correlation section if 3-feature SVM does not have decreased latencey  or better sensitivity or FDR compared with the 5-feature SVM?
\item Need to remove Figure 3?  Yes, since it was derived using the ``new'' method.  Probably not needed for an EE-centric journal only, but should do for a CS journal in future.  
\item ECS: MCOOB, MCD - Tie in to use of SVM.  Use as \textbf{strawman}.  Eduardo to add section tying these into SVM.
\item ECS to develop a Table to show: Severity of decorrelation during spoofing is different than the severity of decorrelation during normal operation.
\item ECS: Table 2 justifying the 5-feature SVM?
\end{itemize}


\section{Notes from 7/15}

\begin{itemize}
\item 3 vs 5 - 5 preferable.  Marginally improved performance if anything. But much faster training, 4 days vs < 1 day.  \hl{Need to remove intra-correlation section?}  Leave it in - points to rational selection of PMU parameters to use.  
\item Prefer 5 over 3 b/c of faster training time.  No advantage gained in sensitivity or computational time in using one or the other.  
\item Intra-cor points towards using V+ mag, V+ angle, f and ROCOF.  Inter-cor suggests first three are good to use, but ROCOF is not.  We use those three as part of the five, and not ROCOF.  ie.  intra-cor analysis is useful, and combined with the inter-cor analysis, we have rationalized our selection of PMU parameters.
\item early labeling versus late labeling.  Initial results looked good, but there may not be enough test data to generalize the SVM well.  But, with full training data sets, results are not so good.  SW Running another experiment: using spoof 9 w/ 5 features, rather than spoof 1.  Justify labeling 'spoof' when window is half full, or just state ``that's what we did!.''  Early timing looks notably better, but does not hold up on the larger data sets.
\item Need more test data?  Not for this EE submission.  
\item Drop heat map figure.
\item Meet again 31st.
\end{itemize}

\section{Notes from 8/6}

\begin{itemize}
\item Eduardo almost done with MCB, MCOOB Figures, to replace Table II.
\item Will plot all five variables from Table II
\item Footnote 4: keep or remove?  Leave it as footnote.  
\item 8 page limit.  Getting close.  
\item Still need to write the conclusion - Xinghui and then Bob 
\item Add bios, Scott and Xinghui and Richard
\item Eduardo to try to shoren the references.
\item Finish all this by Thursday next week, 8/13, meet at 9am.
\end{itemize}

\section{Noted from 8/13}
\begin{itemize}
\item Eduardo to add MCD/MCOOB plot.  Add caption and discussion in body.
\item Did we use 8 or 9 classifiers for the ensemble?
\item Add comment on phi_- and phi-0 in SVM section pertaining to why these two parameters bring value to the analysis.  Within the body, is there already a comment along the lines of ``We have shown that using 5 versus 3 parameters improves the \textbf{training time} of the classifiers.''?
\item all figs in .eps?
\item Eduardo to submit this weekend, Sunday.
\end{itemize}
